Leveraging the Domain Adaptation of Retrieval Augmented Generation Models for Question Answering and Reducing Hallucination

While ongoing advancements in Large Language Models have demonstrated remarkable success across various NLP tasks, Retrieval Augmented Generation Model stands out to be highly effective on downstream applications like Question Answering. Recently, RAG-end2end model further optimized the architecture and achieved notable performance improvements on domain adaptation. However, the effectiveness of these RAG-based architectures remains relatively unexplored when fine-tuned on specialized domains such as customer service for building a reliable conversational AI system. Furthermore, a critical challenge persists in reducing the occurrence of hallucinations while maintaining high domain-specific accuracy. In this paper, we investigated the performance of diverse RAG and RAG-like architectures through domain adaptation and evaluated their ability to generate accurate and relevant response grounded in the contextual knowledge base. To facilitate the evaluation of the models, we constructed a novel dataset HotelConvQA, sourced from wide range of hotel-related conversations and fine-tuned all the models on our domain specific dataset. We also addressed a critical research gap on determining the impact of domain adaptation on reducing hallucinations across different RAG architectures, an aspect that was not properly measured in prior work. Our evaluation shows positive results in all metrics by employing domain adaptation, demonstrating strong performance on QA tasks and providing insights into their efficacy in reducing hallucinations. Our findings clearly indicate that domain adaptation not only enhances the models' performance on QA tasks but also significantly reduces hallucination across all evaluated RAG architectures.

==> agreement.tex <==
\subsection{Agreement}


\subsubsection{Dataset}
In the quality assurance process, six annotators were employed to refine and validate the generated 18,662 QA pairs. The annotators were provided with both the knowledge base and the corresponding QA pairs. Their first task was to evaluate whether each question aligned with the knowledge base and whether it was of high quality. If the question met these criteria, it was retained. Otherwise, the annotators were instructed to rewrite the question.

Once all annotators reviewed the questions, we applied an agreement threshold: if over 50\% of the annotators agreed that the question was valid, we retained it in its original form. In cases where consensus was lacking, we selected the best version of the question from the rewritten suggestions.

Following the validation phase, we analyzed the entire dataset to assess the distribution of question and answer types. If certain types were over-represented, we re-balanced the dataset by regenerating new questions of that type. These newly generated questions were again subjected to the same validation process by the annotators, ensuring both quality and balance across the dataset.




\subsubsection{Hallucination Evaluation}

As earlier discussed, we have created a set of QA pair for evaluating hallucination. After obtaining the model responses, we sent the corresponding QA pairs containing the ground truth and model-generated answers to our annotators for further evaluation. 

The annotators were asked to perform a two-stage categorization as mentioned in the guideline. Initially, they categorized each response as either "Supported," "Non-supported," or "Irrelevant," based on its alignment with the knowledge base. Subsequently, they classified the responses into one of the following finer-grained categories: "Correct," "Bias," "Ambiguous," "Incompleteness," or "Under Informativeness."

Following this dual categorization, we applied a consensus rule: if more than 50\% of annotators assigned the same category, the classification was accepted. In cases where there was insufficient agreement, the responses were re-evaluated internally to ensure accurate categorization. This process was essential in gauging both the model’s performance and the types of hallucination it might generate.
